MAVFI: An End-to-End Fault Analysis Framework with Anomaly Detection and Recovery for Micro Aerial Vehicles

Safety and resilience are critical for autonomous unmanned aerial vehicles (UAVs). We introduce MAVFI, the micro aerial vehicles (MAVs) resilience analysis methodology to assess the effect of silent data corruption (SDC) on UAVs' mission metrics, such as flight time and success rate, for accurately measuring system resilience. To enhance the safety and resilience of robot systems bound by size, weight, and power (SWaP), we offer two low-overhead anomaly-based SDC detection and recovery algorithms based on Gaussian statistical models and autoencoder neural networks. Our anomaly error protection techniques are validated in numerous simulated environments. We demonstrate that the autoencoder-based technique can recover up to all failure cases in our studied scenarios with a computational overhead of no more than 0.0062%. Our application-aware resilience analysis framework, MAVFI, can be utilized to comprehensively test the resilience of other Robot Operating System (ROS)-based applications and is publicly available at https://github.com/harvard-edge/MAVBench/tree/mavfi.

==> 2_Background.tex <==
%\section{Background}
\section{ Motivation and Background}
\label{sec:background}
\vspace{-3pt}
\textbf{Safety standards.} Many efforts have been dedicated to AV safety. The safety standard ISO 26262~\cite{palin2011iso} has been developed to provide guidance and safety requirements for vehicle and their systems. A variety of fault tolerance analyses has been performed for the computing system \cite{jha2019ml,gan2022braum} of AVs. 

Unfortunately, to date, there are no comprehensive standards for \emph{autonomous} UAV assessment. Prior works mainly focus on evaluating learning-based navigation system~\cite{wan2021analyzing}. However, PPC compute paradigm-based UAV system is widely adopted in UAV systems nowadays, and its fault tolerance has not been adequately explored.
Therefore, {we take the first step to explore how SDCs propagate through the entire end-to-end PPC computational pipeline and impact the resilience of UAVs.}

\begin{figure}[t!]
\centering\includegraphics[width=.9\columnwidth]{figs/background/compute_stack_v2.pdf}
        \caption{System stack for a UAV. UAVs are complex cyber-physical systems with strong inter-dependencies between the computing and physical components. We focus on how faults in the companion computer affect the rest of the system.}
        \label{fig:UAV_system}
        \vspace{-10pt}
\end{figure}

\textbf{System Layer.} To understand how to address safety and resilience in UAVs, we must understand their end-to-end system configuration. Fig.~\ref{fig:UAV_system} presents the computing stack of a UAV system. In the system layer, robot operating system (ROS) is used to provide message-passing between processes and resource allocation for robotic applications. ROS consists of multiple nodes, services, and a ROS master to support the functionalities and communications~\cite{quigley2009ros}. Under ROS, Linux maps workloads to compute units and schedules the tasks. %Each ROS node is treated as a process that is scheduled to a thread on CPU cores. % aiming at managing cyber-physical systems by providing services for heterogeneous computing, low-level device control logic, and message-passing between processes.


\textbf{Hardware Layer.} This layer consists of sensors, a companion computer, and a flight controller. 
The companion computer is used to execute the PPC kernels. These kernels usually act as ROS nodes and run on a general-purpose processor (e.g., CPU). Unlike autonomous vehicles, UAVs are limited in computing resources and energy budget, and thus, it is less common to equip UAVs with power-intensive GPU. The companion computer generates high-level flight commands (e.g., velocity in $x$, $y$, $z$ directions) in response to the sensor readings. The flight controller converts the high-level flight commands to low-level actuation commands to control and stabilize the UAV. In this work, we consider the faults in the companion computer. 

%The former determines the flight commands based on the real-time sensor readings, while the latter executes the commands. For instance, a corrupted yaw rotation generated by the companion computer could direct the UAV to point toward an obstacle and cause collisions. Meanwhile, the flight controller only executes the given commands without knowing the world models. 


%\textbf{Algorithms.} There has been significant advancement in perception, localization, mapping, and deep learning~\cite{lynen2015get,liu2016high,krishnan2019air,loquercio2018dronet,krishnan2019quantized,anwar2020autonomous,gao2021ielas,wan2021energy,krishnan2021autosoc}. Among all autonomy paradigms, the PPC computational pipeline is a widely used system \cite{boroujerdian2018mavbench}. In the PPC pipeline, the perception stage takes the sensor data and creates three-dimensional models to provide a volumetric representation of space, such as a point cloud~\cite{rusu20113d} and occupancy map~\cite{fleuret2007multicamera}. The three-dimensional models are then fed into the planning stage to determine a collision-free trajectory by running a motion planner (e.g., RRT~\cite{kuffner2000rrt} and their variants~\cite{motion-planning-survey}). Finally, based on UAV's dynamics, the control stage follows the planned path through PID~\cite{ang2005pid} or other controllers. 





==> Backup.tex <==
\subsection{Anomaly Detection and Recovery}
\vspace{-3pt}
\label{subsec:stage_combination}
% Fig.~\ref{fig:detect_percentage} and Fig.~\ref{fig:detect_stage}
\begin{figure}[b!]
\centering
\vspace{-15pt}
    \subfloat[][Autoencoder-based anomaly detection and recovery.\label{fig:stage_autoencoder}]{\includegraphics[width=0.42\textwidth]{figs/results/recovery_autoencoder.pdf}}
    \vspace{-5pt}
    \caption{Worst-case QoF metrics with different error detection and recovery stages (normalized to golden run).}
    \label{fig:detect_stage}
    %\vspace{-10pt}
\end{figure}



To evaluate error detection effectiveness in different PPC stages, we experiment with the autoencoder-based anomaly detection and recovery scheme for certain compute stages.

\textbf{Single-stage detection and recovery.}
We first experiment the anomaly detection and recovery by only detecting a single pipeline stage. As shown in Fig.~\ref{fig:detect_stage}, the autoencoder-based technique recovers the flight time by 20.1\%, 59.3\%, and 73.2\% for perception, planning, and control, respectively, along with the success rate improvement, in \textit{Factory} environment. A similar trend has been demonstrated in the other three environments. The flight time can be recovered the most by detecting the faults that happened in the control stage. The reasons are twofold. First, the planning and control stages are more vulnerable to faults from the system perspective. Second, any error propagated from previous stages has to pass through the control stage before corrupting the flight command. 

\textbf{Multi-stage detection and recovery.}
To understand how different stages affect the anomaly detection and recovery, we apply the scheme to multi-stages, namely the planning-and-control (PC) stage and all PPC stages. The flight time recovers by 74.8\%, 87.1\% for PC and PPC, respectively, along with the success rate increase, in \textit{Factory} environment. Detecting PC stage achieve slightly better performance than only detecting control in \textit{Factory}, \textit{Farm}, and \textit{Sparse} environment. However, in \textit{Dense} environment, detecting the PC stage greatly outperforms detecting the control stage by 47.4\%. 
These results indicate that a UAV achieves similar or higher performance by monitoring more stages, and the performance benefit is more for complex environments. 

==> tab/MAVFI_compare.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table*}[t!]
\vspace{-0.15in}
\centering
\caption{Comparison between ROSFI and prior fault injection methods.}
\vspace{-3pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c||c|c|c|c|c||c|}
\hline
\textbf{}          & \textbf{LLFI}~\cite{lu2015llfi} & \textbf{PINFI}~\cite{wei2014quantifying} & \textbf{CLEAR}~\cite{cheng2016clear} & \textbf{SASSIFI}~\cite{hari2017sassifi} & \textbf{DriveFI}~\cite{jha2019ml} & \textbf{ROSFI (This work)} \\ \hline
Autonomous Vehicle &  {\color{red}\xmark}     &  {\color{red}\xmark}      &  {\color{red}\xmark}      &  {\color{red}\xmark}        & {\color{green}\cmark}(Vehicle) & {\color{green}\cmark}(Drone) \\ \hline 
Support ROS   &  {\color{red}\xmark}        & {\color{red}\xmark}          &  {\color{red}\xmark}       &  {\color{red}\xmark}         &  {\color{red}\xmark}         & {\color{green}\cmark}\\\hline
Platform  & CPU & CPU  & CPU    & GPU   & GPU          & CPU             \\ \hline\hline
Injection level    & IR-level      & Instruction-level & RLT-level      & Instruction-level   & Instruction-level, Source-level   & Instruction-level, Source-level             \\\hline
Single Bit-flip          & {\color{green}\cmark}& {\color{green}\cmark}& {\color{green}\cmark}& {\color{green}\cmark}& {\color{green}\cmark}& {\color{green}\cmark}\\ \hline
Double Bit-flips          & {\color{green}\cmark}& {\color{red}\xmark}& {\color{red}\xmark}& {\color{green}\cmark} & {\color{green}\cmark}& {\color{green}\cmark}\\ \hline
Multiple Bit-flips          & {\color{red}\xmark}& {\color{red}\xmark}& {\color{red}\xmark}& {\color{red}\xmark}& {\color{green}\cmark}& {\color{green}\cmark}\\ \hline 
\end{tabular}
}
% \caption{Comparison between ROSFI and prior fault injection methods.}
\label{tab:ROSFI_compare}
\end{table*}

==> tab/detection_compare.tex <==
\renewcommand{\arraystretch}{1.2}

\begin{table}[t!]
\centering
\vspace{-5pt}
\caption{Properties of anomaly detection techniques.}
\vspace{-5pt}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Techniques}          & \begin{tabular}[c]{@{}l@{}}\textbf{Training} \\ \textbf{required}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Initialization}\\ \textbf{dataset}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Computation}\\ \textbf{overhead}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Detection}\\ \textbf{effectiveness}\end{tabular} \\ \hline
Autoencoder (This work)          & Unsupervised                                                 & Large                                                             & Large                                                          & Good                                                         \\ \hline
Neural network based & Supervised                                                   & Large                                                             & Large                                                          & Good                                                              \\ \hline
Clustering based     & No                                                           & Moderate                                                          & Moderate                                                       & Moderate                                                            \\ \hline
Gaussian model (This work)    & No                                                           & Moderate                                                          & Low                                                            & Moderate                                                            \\ \hline
\end{tabular}
}
% \caption{Properties of anomaly detection techniques.} 
\label{tab:detect_comparison}
\vspace{-5pt}
\end{table}

==> tab/i9_TX2.tex <==
\renewcommand{\arraystretch}{1.2}

\begin{table}[]
\centering
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{|l|l|l|}
\hline
                     & \textbf{Intel i9} & \textbf{TX2} \\ \hline
Core numbers         & 14                & 4            \\ \hline
Core frequency (GHz) & 3.3               & 2            \\ \hline
Power (Watt)         & 165               & 7.5          \\ \hline
Flight time (s)      & 115               & 322          \\ \hline
Flight energy (kJ)   & 61.7              & 177.1        \\ \hline
\end{tabular}
}
\end{table}

==> tab/multi-bit.tex <==
% \begin{table}[t!]
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \textbf{Bit Flips}  & \textbf{\begin{tabular}[c]{@{}c@{}}Flight\\ Time (s)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Flight\\ Distance (m)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Total\\ Energy (kJ)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Number of\\ Re-plans\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Success\\ Rate (\%)\end{tabular}} \\ \hline
% \textbf{0 (golden)} & 94.6                                                               & 49.5                                                                   & 51.4                                                                 & 3.71                                                                  & 100                                                                  \\ \hline
% \textbf{1}          & 105.6                                                              & 55.9                                                                   & 57.2                                                                 & 4.07                                                                  & 92                                                                   \\ \hline
% \textbf{3}          & 107.3                                                              & 56.8                                                                   & 58.7                                                                 & 4.19                                                                  & 91                                                                   \\ \hline
% \textbf{5}          & 111.8                                                              & 59.4                                                                   & 61.1                                                                 & 4.28                                                                  & 89                                                                   \\ \hline
% \end{tabular}
% \end{table}

\renewcommand{\arraystretch}{1.2}
\begin{table}[h!]
\vspace{-10pt}
\centering
\caption{QoF metrics with different number of bit-flip injections.}
% \vspace{-2pt}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Bit Flips}  & \textbf{\begin{tabular}[c]{@{}c@{}}Flight\\ Time (s)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Flight\\ Distance (m)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Total\\ Energy (kJ)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Number of\\ Re-plans\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Success\\ Rate (\%)\end{tabular}} \\ \hline
\textbf{0 (golden)} & 94.6                                                               & 49.5                                                                   & 51.4                                                                 & 3.71                                                                  & 100                                                                  \\ \hline
\textbf{1}          & 105.6                                                              & 55.9                                                                   & 57.2                                                                 & 4.07                                                                  & 92                                                                   \\ \hline
\textbf{3}          & 107.3                                                              & 56.8                                                                   & 58.7                                                                 & 4.19                                                                  & 91                                                                   \\ \hline
\textbf{5}          & 111.8                                                              & 59.4                                                                   & 61.1                                                                 & 4.28                                                                  & 89                                                                   \\ \hline
\end{tabular}
}
% \caption{The MAV performance impact with injection of single and multiple bit-flips.}
\label{tab:multi-bit}
\vspace{-15pt}
\end{table}

==> tab/overview_compare.tex <==
\renewcommand{\arraystretch}{1.5}

\begin{table}[]
\caption{Fault characteristics of autonomous vehicles.}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|l|l|l|}
\hline
                         & Sensor & Perception & Planning & Control \\ \hline
\textbackslash{}cite\{\} & v      &           &          &         \\ \hline
\textbackslash{}cite\{\} & v      & v         &          &         \\ \hline
Our work                 &        & v         & v        & v       \\ \hline
\end{tabular}
}
% \caption{Fault characteristics of autonomous vehicles.}
\label{tab:fault overview}
\end{table}

==> tab/variable.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \renewcommand*{\arraystretch}{1}
% \resizebox{0.8\linewidth}{!}{
% \tiny
% \begin{tabular}{c|c|c}
% \hline
% \textbf{Stage (Algorithm)}            & \textbf{Variable Datatype} & \textbf{Variable Name}      \\ \hline
% \multirow{3}{*}{Perception (Octomap)} & float64                    & time\_to\_collision         \\
%                                       & float64                    & future\_collision\_sequence \\
%                                       & bool                       & collision                   \\ \hline
% \multirow{10}{*}{Planning (RRT)}      & float64                    & x, y, z                     \\
%                                       & float64                    & vx, vy, vz                  \\
%                                       & float64                    & ax, ay, az                  \\
%                                       & float64                    & yaw                         \\
%                                       & bool                       & blocking\_yaw               \\
%                                       & float64                    & duration                    \\
%                                       & bool                       & append                      \\
%                                       & bool                       & reverse                     \\
%                                       & float64                    & trajectory\_sequence        \\
%                                       & float64                    & future\_collision\_sequence \\ \hline
% \multirow{3}{*}{Control (PID)}        & float64                    & vx, vy, vz                  \\
%                                       & float64                    & duration                    \\
%                                       & float64                    & yaw\_rate                   \\ \hline
% \end{tabular}
% }
% \caption{Representative cross-stage variables are selected for fault injection experiments.}
% \label{tab:variable}
% \end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\renewcommand*{\arraystretch}{1.2}
\resizebox{0.9\linewidth}{!}{
\tiny
\begin{tabular}{|c|c|c|}
\hline
\textbf{Stage}            & \textbf{Variable Datatype} & \textbf{Variable Name}      \\ \hline
\multirow{Perception} & float64                    & time\_to\_collision         \\ \cline{2-3} 
                                      & float64                    & future\_collision\_sequence \\ \cline{2-3} 
                                      & bool                       & collision                   \\ \hline
\multirow{Planning}      & float64                    & x, y, z                     \\ \cline{2-3} 
                                      & float64                    & vx, vy, vz                  \\ \cline{2-3} 
                                      & float64                    & ax, ay, az                  \\ \cline{2-3} 
                                      & float64                    & yaw                         \\ \cline{2-3} 
                                      & bool                       & blocking\_yaw               \\ \cline{2-3} 
                                      & float64                    & duration                    \\ \cline{2-3} 
                                      & bool                       & append                      \\ \cline{2-3} 
                                      & bool                       & reverse                     \\ \cline{2-3} 
                                      & float64                    & trajectory\_sequence        \\ \cline{2-3} 
                                      & float64                    & future\_collision\_sequence \\ \hline
\multirow{Control}        & float64                    & vx, vy, vz                  \\ \cline{2-3} 
                                      & float64                    & duration                    \\ \cline{2-3} 
                                      & float64                    & yaw\_rate                   \\ \hline
\end{tabular}
}
\caption{Representative cross-stage variables are selected for fault injection experiments.}
\label{tab:variable}
\end{table}
